Branching laws for small unitary representations of GL(n,C)

The unitary principal series representations of $G=GL(n,\mathbb{C})$ induced from a character of the maximal parabolic subgroup $P=(GL(1,\mathbb{C})\times GL(n-1,\mathbb{C}))\ltimes\mathbb{C}^{n-1}$ attain the minimal Gelfand--Kirillov dimension among all infinite-dimensional unitary representations of $G$. We find the explicit branching laws for the restriction of these representations to symmetric subgroups of $G$.

==> preambel.tex <==
\usepackage[T1]{fontenc}
\usepackage[ngerman,english]{babel}
\usepackage{amsmath}
\usepackage{amsthm}
\usepackage{amssymb}
\usepackage{amsfonts}
\usepackage{amsxtra}
\usepackage{color}
\usepackage[breaklinks]{hyperref}
\usepackage{enumitem}
\usepackage{tocloft}
\usepackage{makeidx}
\usepackage{textcomp}
\usepackage{tabularx}
\usepackage{rotating}
\usepackage{multirow}
\usepackage{booktabs,longtable}
\usepackage[all]{xy}
\usepackage{float}

\setenumerate{itemsep=0pt} % topsep=0pt
\setitemize{itemsep=0pt} % topsep=0pt
\setdescription{itemsep=0pt} % topsep=0pt
\setlist{noitemsep}
%\setlength{\itemsep}{0pt}
%\setlength{\parskip}{0pt}
%\setlength{\parsep}{0pt}
%\addtolength{\cftbeforesecskip}{-9pt}
%\renewcommand{\cftsecfont}{\normalfont}

\makeindex

\setcounter{tocdepth}{2}

